Demystifying the Data Need of ML-surrogates for CFD Simulations

Computational fluid dynamics (CFD) simulations, a critical tool in various engineering applications, often require significant time and compute power to predict flow properties. The high computational cost associated with CFD simulations significantly restricts the scope of design space exploration and limits their use in planning and operational control. To address this issue, machine learning (ML) based surrogate models have been proposed as a computationally efficient tool to accelerate CFD simulations. However, a lack of clarity about CFD data requirements often challenges the widespread adoption of ML-based surrogates among design engineers and CFD practitioners. In this work, we propose an ML-based surrogate model to predict the temperature distribution inside the cabin of a passenger vehicle under various operating conditions and use it to demonstrate the trade-off between prediction performance and training dataset size. Our results show that the prediction accuracy is high and stable even when the training size is gradually reduced from 2000 to 200. The ML-based surrogates also reduce the compute time from ~30 minutes to around ~9 milliseconds. Moreover, even when only 50 CFD simulations are used for training, the temperature trend (e.g., locations of hot/cold regions) predicted by the ML-surrogate matches quite well with the results from CFD simulations.

==> 0-abstract.tex <==
%
%
%quite 
% Our team tested the accuracy of the neural network prediction with the actual CFD simulation results and found that the results from both techniques matched well for 100XXX????, 500, 1000, 1500 and 2000 data samples. Our team also tested the prediction model based on 50 data samples (E-tiny) and found that the prediction of the temperature trend (hot and cold zones) matched with the CFD results, but variation in the magnitude of the temperature on the surface was observed.
% we have coupled the machine learning algorithm with Computational Fluid Dynamics (CFD) to predict . CFD model was used to generate CFD data by carrying out CFD simulations  for  in the cabin. 
% in particular, the number of high-fidelity CFD simulation the amount of data needed for training the machine learning models are essential for the successful use of surrogate models for prediction of flow properties like temperature, pressure, heat transfer and aerodynamic coefficients.
% and techniques to extract key performance indexes from the CFD data for the surrogate models to achieve the desired objectives have been a challenge.  
% Last few years have witnessed a significant interest in using surrogate models as a complimentary tool along with CFD models for predicting flow properties. 
% Understanding the 
% In this study, we have coupled the machine learning algorithm with Computational Fluid Dynamics (CFD) to predict the temperature distribution inside the passenger vehicle cabin. CFD model was used to generate CFD data by carrying out CFD simulations  for various operating conditions in the cabin. 
%\krishna{Biswa please include ML techniques description as needed and confirm the data samples that was used for the surrogate model}. 
% While the team tested the application of 100 (Expt.xxxxx),500 (Expt.1), 1,000 (Expt.2), 1,500 (Expt.3), and 2,000 (Expt.4) data samples to train the network, the prediction error was observed to remain stable. Our team tested the accuracy of the neural network prediction with the actual CFD simulation results and found that the results from both techniques matched well for 100XXX????, 500, 1000, 1500 and 2000 data samples. Our team also tested the prediction model based on 50 data samples (E-tiny) and found that the prediction of the temperature trend (hot and cold zones) matched with the CFD results, but variation in the magnitude of the temperature on the surface was observed.
%
%
%
%
% https://media.plm.automation.siemens.com/simcenter/flipbook-new-8/ei8/if-i-dont-use-ai-am-i-really-an-engineer/}
